A General and Configurable Framework for Blockchain-based Marketplaces

The first generation of blockchain focused on digital currencies and secure storage, management and transfer of tokenized values. Thereafter, the focus has been shifting from currencies to a broader application space. In this paper, we systematically explore marketplace types and properties, and consider the mechanisms required to support those properties through blockchain. We propose a generic and configurable framework for blockchain-based marketplaces, and describe how popular marketplace types, price discovery policies, and other configuration parameters are implemented within the framework by presenting concrete event-based algorithms. Finally, we consider three use cases with widely diverging properties and show how the proposed framework supports them.

==> algorithms/algoValidation.tex <==

%
%   NOT FINALIZED
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% VALIDATION ALGORITHM
\begin{algorithm*}
\caption{Block validation by node $n$}

% \SetKwFunction{isOddNumber}{isOddNumber}
\SetKwInput{Input}{Input}
% \SetKwInput{Output}{Output}
% \SetKwInOut{KwIn}{Input}
% \SetKwInOut{KwOut}{Output}
\KwIn{block B}
% \KwOut{winning bid}


\SetKwProg{Fn}{func}{ : }{}
\Fn{validateBlock}{
    \ForEach{\rm item advertisement $A$ received from the network and included in $B$}{
        \If{\rm \textit{A.tType} is not a valid type}{
            \KwRet false
        }
        \If{\rm $A.\delta_{\rm{sale}}$ is longer than admissible duration by the marketplace}{
            \KwRet false
        }
        \If{\rm \textit{A.revFlag} is not valid}{
            \KwRet false
        }
        \If{\rm \textit{A.F} is not valid}{
            \KwRet false
        }
        \tcp{Optional inputs are left out of the pseudo-code scope}
    }
    
    \ForEach{\rm \textit{bid} received from the network and included in $B$}{
    
    \textit{bidBlockNum} $\leftarrow$ {number of block $B$} \\
    
    \textit{adBlock} $\leftarrow$ {block stored in the blockchain that includes $A$} \\
    \textit{adBlockNum} $\leftarrow$ {number of block \textit{adBlock}} \\
    
    %\textit{adBids} $\leftarrow \{\textit{bid}\, | \textit{bid}$ is for $A$ $\land$ \textit{bid} $\in$ a block stored in blockchain between \textit{adBlock} and $B$\} \\
    
    \If{\rm (\textit{bid.A} is not defined) $\lor$ (\textit{bid.C} is not defined)}{
        \KwRet false
    }
    
    \eIf{bidBlockNum < adBlockNum + A.$\delta_{\rm{sale}}$}{
        
        \textit{lastBid} $\leftarrow$ last \textit{bid} for $A \in$ a block stored in blockchain between $B$ and \textit{adBlock}  
        
        \textit{lastBidBlockNum} $\leftarrow$ number the block containing \textit{lastBid}
        
        \If{\rm \textit{lastBid} $\land$ \textit{lastBidBlockNum} are defined}{
        
            \Switch{A.tType}{
            \Case{english auction}{
                
                \If{\rm \textit{bid.P} is not defined}{
                    \KwRet false
                }
                
                \textit{prevBidsForA} $\leftarrow$ \{\textit{prevBid} | \textit{prevBid} is for $A$ $\land$ \textit{bid} $\in$ is included in the blockchain between $A$ and \textit{bid} \}\\
            

                \If{\rm \textit{prevBidsForA} $\neq \emptyset$}{
                    \textit{highestBid} $\leftarrow \textit{max}_{\textit{bid} \in \textit{prevBidsForA}} |\textit{bid}.P| $ \\
                    
                    \If{\rm \textit{bid.P} $<$ \textit{highestBid}}{
                        \KwRet false
                    }
                }
                    
                \If{\rm  (\textit{bid.P} $-$ \textit{A.stPrice})$\mod A.\Delta_{\rm{bid}} = 0$}{
                    \tcc{Increment is quantized}
                    \KwRet false
                }
                
                %\If{$lastBidBlockNum + A.\delta_{\rm{bid}} < bidBlockNum$}{
                
                %    \If{\rm \textit{bid.P} $<$ \textit{lastBid.P}}{
                 %       \KwRet false
                 %   }
                %}
                
                %\If{bid.P = highest bid or highest bid.P times }{}
                

                }
                \Case{dutch auction}{
                
                    \If{\rm \textit{bid.P} is not defined}{
                        \KwRet false
                    }
                    
                    \textit{prevBidsForA} $\leftarrow$ \{\textit{prevBid} | \textit{prevBid} is for $A$ $\land$ \textit{bid} $\in$ is included in the blockchain between $A$ and \textit{bid} \}\\
                    
                    \uIf{\rm \textit{prevBidsForA} $\neq \emptyset$ \, $\land$ |\textit{bid.P}| $\neq$ |\textit{prevBidsForA.P}| }{
                        \KwRet false
                    }
                    \uElseIf{\rm \textit{prevBidsForA} $= \emptyset$}{
                        \textit{currValidPr} $= A.stPrice - \lfloor \frac{bidBlockNum - adBlockNum}{A.\delta_{\rm{bid}}} \rfloor A.\Delta_{\rm{bid}}$
                        
                        
                        \If{\rm |\textit{bid.P}| $\neq$ \textit{currValidPr}}{
                            \KwRet false
                        }
                    }
                }
                \Case{committee-based eval and ranking}{
                    \textit{validateBidContent(bid.C)}
                }
                \Case{committee-based eval and custom objective ranking}{
                    \textit{validateBidContent(bid.C)}
                }
                \Case{custom objective eval and ranking}{
                    \textit{validateBidContent(bid.C)}
                }
            }
        }
    }{
        \tcp{The bidding time for the traded item in A has expired}
        \KwRet false
    }
    }
    
    \ForEach{\rm bid evaluation (A, b, C) received from the network and included in B}{
        \uIf{bid evaluation sender is \textbf{not} in A.evalCom}{
            \KwRet false
        }
        \uElseIf{bid evaluation does not point to a valid bid}{
            \KwRet false
        }
        \Else{
            validate bid evaluation
        }
    }
    
    \ForEach{\rm item assignment (A, b, be) received from the network and included in B}{
        {validate item assignment}
    }
    
    \ForEach{\rm revelation (A) received from the network and included in $B$}{
        
        resPrice $\leftarrow$ revelation\\
        
        \If{\rm resPrice does not match A.resPHash}{
            \KwRet false
        }
        %{validate revelation}
    }
    
\textbf{return} \textit{true}
}
\end{algorithm*}

==> table3.tex <==
%%%%%%%%%%%%%%%%%%%%%%% ----- TABLE -------
\begin{table*}[ht!!!]

\tabcolsep 5pt
\normalsize
\centering
		
	\caption{Parameters configuration for the use cases}
		
		\begin{tabular}{p{3cm} p{4cm} p{4cm} p{4cm}}
			
		\toprule
		  \bf Parameter & 
		  \bf Physical goods &  
		  \bf Logo design contest &
		  \bf Job posting \\
		\toprule
	    
	    {\it{\specialcell[t]{Trading item\\and metadata}}} &
		Generic physical goods. 
		& 
		Contest rules. 
		& 
		Job position.
		\\
		
		\toprule
		
		{\it \specialcell[t]{Trade type}} &
		English auction. 
		&
		Committee-based eval and custom objective ranking. 
		&
		Committee-based eval and ranking. \\
		
		\toprule
		
		{\it \specialcell[t]{Bid evaluation\\ and matching}} 
		&
		Objective.
		%Bidding values increment monotonically. If the bid is not challenged for an established number of blocks, the item is assigned to the last bid proposer. Otherwise, if a higher bid is placed, the countdown (measured in number of blocks) is refreshed. New bids are subject to a minimum increase to be considered valid.
        & 
        Subjective.
        & Subjective. \\
        
        %The proposer of the winning logo is compensated according to the advertised reward. 
	    
	    \toprule
		
		
		{\it \specialcell[t]{Selection of the\\evaluation committee}} &
		None. 
		&
		Authorized experts.
		& 
		Selected examiners. \\
		%in a pseudo-random fashion with reinsertion, so that they can be re-extracted for additional evaluations.
		
		
		\toprule
		

	    
     {\it \specialcell[t]{Money and\\item flow}} & 
     On-chain. 
     &  
     On-chain. 
     & 
     Off-chain.  \\
 
 	\toprule
 	
     {\it \specialcell[t]{Duration and time}} 
     & 
     1--10 days.
     & 
     14 days.
     & 
     Three weeks.
     \\
     
	\toprule
	
	\end{tabular}
	
	\label{tab:results}
	\end{table*}
